Re-Examine Distantly Supervised NER: A New Benchmark and a Simple Approach

Distantly-Supervised Named Entity Recognition (DS-NER) uses knowledge bases or dictionaries for annotations, reducing manual efforts but rely on large human labeled validation set. In this paper, we introduce a real-life DS-NER dataset, QTL, where the training data is annotated using domain dictionaries and the test data is annotated by domain experts. This dataset has a small validation set, reflecting real-life scenarios. Existing DS-NER approaches fail when applied to QTL, which motivate us to re-examine existing DS-NER approaches. We found that many of them rely on large validation sets and some used test set for tuning inappropriately. To solve this issue, we proposed a new approach, token-level Curriculum-based Positive-Unlabeled Learning (CuPUL), which uses curriculum learning to order training samples from easy to hard. This method stabilizes training, making it robust and effective on small validation sets. CuPUL also addresses false negative issues using the Positive-Unlabeled learning paradigm, demonstrating improved performance in real-life applications.

==> sections/2related.tex <==
\section{Related Work}\label{sec:related}
% Fully supervised NER using deep neural networks always requires a large number of training data with human annotations, which is very costly. To alleviate the human efforts on annotating, DS-NER has been proposed and received increasing research interest recently, where annotations can be obtained from existing professional dictionaries or knowledge bases by some matching or query methods. However, because of the polysemy in language and the limited coverage of distant supervision resources, DS-NER often suffers from annotation errors like false positive, false negative, and positive type errors. Therefore, handling annotation errors in DS-NER has drawn special attention 

\subsection{Benchmark Datasets}
To reduce the cost of human-annotated training data for NER tasks, DS-NER uses professional dictionaries or knowledgebases for annotations. Existing DS-NER benchmark datasets use NER benchmark datasets to simulate the distant supervision setting by replacing the human annotations on training datasets with knowledge base annotations \cite{liang2020bond, shang2018learning, zhou2022distantly}. There are some potential biases of current DS-NER benchmarks. 1) Only BC5CDR \cite{shang2018learning} dataset comes from professional domains where DS-NER tasks are in high demand. 2) A series of hand-crafted procedures were applied to the current DS-NER benchmarks. Such procedures are entity-type dependent and require substantial human effort, and thus may not be generalizable to other DS-NER tasks. 3) The major entity types in existing DS-NER benchmarks consist of many proper nouns (such as person's names, location, and gene names), but in many applications, the entities to recognize need not be proper nouns. 


\subsection{DS-NER Methods}

Handling annotation errors in DS-NER tasks has drawn special attention. Here we briefly discuss a few representative approaches. 
%\cite{yang2018distantly, shang2018learning, mayhew2019named, cao2019low, peng2019distantly, liang2020bond, liu2021noisy, zhang2021biasing, zhang2021improving, meng2021distantly}. 

One line of work assumes that distant supervision often has high-quality positive labels, therefore focusing on alleviating the impact of false negative errors. Some methods address this issue by detecting potential entity candidates \cite{shang2018learning, xu-etal-2023-sampling}.
%AutoNER \cite{shang2018learning} proposes a new tagging scheme to identify entity candidates and does not count the training loss on those candidates.
% \citet{mayhew2019named} introduce a constraint-driven iterative algorithm learning to detect false negative errors in the noisy data and down-weigh them, resulting in a weighted training set on which a weighted NER model is trained. Top-Neg \cite{xu-etal-2023-sampling} selectively uses negative samples with high similarity to positives of the same entity type, improving performance by effectively distinguishing false negatives. 
Some methods adopt positive and unlabeled learning to tackle false negative errors from the loss estimation perspective without separate detection steps \cite{peng2019distantly,zhou2022distantly}. Due to its superiority in tolerating false negative errors, we embed Conf-MPU \cite{zhou2022distantly} into our proposed method.
 

Another line of work simultaneously considers annotation errors of all types. 
% \citet{cao2019low} design a data selection scheme to compute scores for annotation confidence and annotation coverage to distinguish high-quality sentences from noisy ones. 
Some methods propose to train an initial model and apply a self-training framework to reduce the impact of noise \cite{liang2020bond, liu2021noisy, zhang2021improving, 10.1609/aaai.v37i11.26583_atsen,li-etal-2023-class}. 
%BOND \cite{liang2020bond}, leveraging the power of the pre-trained language model RoBERTa, first adopts early stopping to prevent overfitting to noisy labels. But it can learn noise before the early stop. \citet{liu2021noisy} propose a calibrated confidence estimation approach for DS-NER and integrate it in an LSTM-CRF model under a self-training framework to reduce the impact of noise. %\citet{zhang2021biasing} study the noise in DS-NER from the perspective of dictionary bias. 
%SCDL \cite{zhang2021improving} takes two teacher-student networks and a co-training paradigm to cope with noise and take full advantage of mislabeled samples. ATSEN \cite{10.1609/aaai.v37i11.26583_atsen} further develops the teacher-student networks and achieves better performance. 
%Methods such as SCDL \cite{zhang2021improving} and ATSEN \cite{10.1609/aaai.v37i11.26583_atsen} aim to detect noise by teacher-student networks, but the students can learn noise and transfer it to the teacher through EMA.
%RoSTER \cite{meng2021distantly} proposes a noise-robust learning scheme consisting of a new loss function and a noisy label removal step to better model training with noisy data. SANTA \cite{si-etal-2023-santa} deals with explicit and implicit errors separately. 
% RoSTER and SANTA aim to reduce the impact of noise through noise-robust loss functions, but this process is inevitably affected by noise
Methods such as RoSTER \cite{meng2021distantly} and SANTA \cite{si-etal-2023-santa} endeavor to diminish noise effects using loss functions tailored for noise resilience. % yet their processes are unavoidably influenced by noise.
%CLIM \cite{li-etal-2023-class} addresses the imbalance problem in different classes with high-quality candidate selection and label generation. 

%CuPUL differs from traditional approaches by adopting Curriculum Learning (CL), which involves initially learning from easier samples. This strategy helps to avoid label noise at the outset, thereby making the model more robust.
These DS-NER approaches obtain promising performance on existing DS-NER benchmark datasets. However, in a real-life DS-NER application, we observe that they fail to obtain satisfactory performances. These methods are trained on noisy labels initially, so the noise detection may have unknown biases and cause irreparable damage.
